An Iris for Expected Cost Analysis

We present ExpIris, a separation logic framework for the (amortized) expected cost analysis of probabilistic programs. ExpIris is based on Iris, parametric in the language and the cost model, and supports both imperative and functional languages, concurrency, higher-order functions and higher-order state. ExpIris also offers strong support for correctness reasoning, which greatly eases the analysis of programs whose expected cost depends on their high-level behavior. To enable expected cost reasoning in Iris, we build on the expected potential method. The method provides a kind of "currency" that can be used for paying for later operations, and can be distributed over the probabilistic cases whenever there is a probabilistic choice, preserving the expected value due to the linearity of expectations. We demonstrate ExpIris by verifying the expected runtime of a quicksort implementation and the amortized expected runtime of a probabilistic binary counter.

==> Environments.tex <==
\newlength{\blockindent}
\setlength{\blockindent}{8mm}

\theoremstyle{coqtheorem}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{theorem}[lemma]{Theorem} %Uncomment this line if you want to use usual theorems from ntheorem
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{exercise}[lemma]{Exercise}

%% Beweise
\theoremstyle{nonumberplain}
\theorembodyfont{\normalfont}
\theoremsymbol{\qed}
\newtheorem{proof}{Proof}
\providecommand*{\toclevel@proof}{0}
\theoremclass{LaTeX}

==> Macros.tex <==
%% Macros

\newcommand{\dg}[1]{\textcolor{blue}{DG: #1}}
\newcommand{\M}[1]{\ensuremath{\textit{#1}}} % \mathup
\newcommand{\imp}{\mathbin{\rightarrow}~}
\newcommand{\Imp}{\mathbin{\Rightarrow}~}
\renewcommand{\iff}{\mathbin{\leftrightarrow}}
\newcommand{\defeq}{\mathrel{\mathop:=}}

\newcommand{\dd}[2]{\ensuremath{#1_1,\dots,#1_{#2}}}  % x_1,...,x_n
\newcommand{\ddd}[2]{\ensuremath{#1_1\dots\,#1_{#2}}}  % x_1...x_n
\newcommand{\col}{\colon}
%\newcommand{\set}[1]{\ensuremath{\{#1\}}}
\newcommand{\mset}[2]{\set{\,#1\mid#2\,}}
\newcommand{\eset}{\ensuremath{\emptyset}}
%\newcommand{\incl}{\ensuremath{\subseteq}}
\newcommand{\bnfor}{~|~} %|
\newcommand{\qedsq}{\hfill\ensuremath{_\blacksquare}}


\newcommand{\logicName}{ExpIris}

\newcommand{\highlight}[1]{\colorbox{yellow}{$\displaystyle #1$}}
\newcommand{\pota}{p}
\newcommand{\potb}{\mathfrak{P}}
\newcommand{\pot}{p}
\newcommand{\cost}{c}
\newcommand{\expecCost}{expecCost}
%\newcommand{\wpP}[][3]{\$#1~ \wpre{#2}{#3} }
\newcommand{\supp}[1]{supp(#1)}
\newcommand{\distr}{\mu}
\newcommand{\distrf}{\kappa}
\newcommand{\bind}[2]{bind(#1, #2)} 
\newcommand{\dirac}[1]{\delta_{#1}}
\newcommand{\pcost}[2]{\mathbb{E}C_{#2}(#1)}

\usepackage{lmodern}
\usepackage{etoolbox}
\expandafter\patchcmd\csname \string\lstinline\endcsname{%
  \leavevmode
  \bgroup
}{%
  \leavevmode
  \ifmmode\hbox\fi
  \bgroup
}{}{%
  \typeout{Patching of \string\lstinline\space failed!}%
}

\lstdefinelanguage{mylang}{
    morekeywords={true, false, rec, inl, inr, if, then, else, fst, snd, match, with, end, AllocN, Free, CmpXchg, Xchg, FAA, fork, tick, ChooseUniform, ChooseWeighted},
    %sensitive,%
    %morecomment=[s]{(*}{*)},%
    morestring=[d]",%
}

\lstset{basicstyle=\ttfamily\normalsize, columns=fullflexible}

\newcommand{\mcode}[1]{\lstinline[language=mylang]!#1!}

\NewDocumentCommand\wpP{m O{} m O{} m}%
{\$#1~ \textlog{wp}^{#2}_{#4}\spac #3 \spac{\left\{#5\right\}}}

\newcommand{\blankpage}{\newpage
\thispagestyle{empty}
\mbox{}
\newpage}

\renewcommand\qed {{% set up
\parfillskip=0pt % so \par doesnt push \square to left
\widowpenalty=10000 % so we dont break the page before \square
\displaywidowpenalty=10000 % ditto
\finalhyphendemerits=0 % TeXbook exercise 14.32
%
% horizontal
\leavevmode % \nobreak means lines not pages
\unskip % remove previous space or glue
\nobreak % don't break lines
\hfil % ragged right if we spill over
\penalty50 % discouragement to do so
\hskip.2em % ensure some space
\null % anchor following \hfill
\hfill % push \square to right
$\square$% % the end-of-proof mark
%
% vertical
\par}} % build paragraph

\newcommand{\eg}{e.g.}


==> acknowledgements.tex <==
I thank all my friends. \todo{Find friends.}

%%% Local Variables:
%%% TeX-master: "thesis"
%%% End:



==> header.tex <==
\makeatletter

% Packages needed
\usepackage[utf8]{inputenc}
\usepackage{geometry}
\usepackage[small,compact]{titlesec}
\usepackage[final]{listings}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{tipa}
\usepackage[english]{babel}
\usepackage{lstautogobble}
%\usepackage{proof}
\usepackage{bussproofs}
\usepackage{needspace}
\usepackage{xspace}
\usepackage[amsmath,hyperref,thmmarks]{ntheorem}
\usepackage{parskip}
\usepackage{scrextend}
\usepackage{wrapfig}
\usepackage[nottoc]{tocbibind}
\usepackage{caption}
\usepackage{coqtheorem}
\usepackage{stmaryrd}
 \usepackage{mathpartir}
\RequirePackage[centercolon]{mathtools}

% For the font
%\usepackage[T1]{fontenc}
%\usepackage{tgpagella}
%\usepackage[euler-digits,small]{eulervm}
%\linespread{1.025}              % Palatino leads a little more leading

\usepackage{fancyhdr}
\usepackage[obeyDraft]{todonotes}
\setlength{\marginparwidth}{3cm}

\usepackage[toc]{glossaries}
\usepackage{natbib}
\bibpunct{[}{]}{,}{n}{,}{;}


\usepackage{iris}
\usetikzlibrary{fit}
\usetikzlibrary{positioning}

\usepackage{heaplang}

\usepackage{pftools}

\usepackage{semantic}

\usepackage{xparse}
\usepackage{xifthen}

%\usepackage[breaklinks, draft=false, pdfusetitle]{hyperref}

\newenvironment{pfoutline}{\begin{array}{l r}\text{We have:} & \text{To show:} \\}{\end{array}}
% Because we use an array, we have to use weird "expandable" commands...
\DeclareExpandableDocumentCommand\pfhave{m}%
  {\multicolumn{2}{l}{#1\hspace{3em}}\\}
\DeclareExpandableDocumentCommand\pfshow{m}%
  {\multicolumn{2}{r}{\hspace{5em}#1}\\}
\DeclareExpandableDocumentCommand\pfhaveshow{m m}%
  {\multicolumn{1}{l}{#1\hspace{5em}}&%
   \multicolumn{1}{r}{#2}\\}
\DeclareExpandableDocumentCommand\pftext{m}%
  {\multicolumn{2}{l}{\text{#1}\hspace{5em}}\\}

\newenvironment{spfoutline}{\begin{array}{l r}\text{Context:} & \text{Goal:} \\}{\end{array}}



\input{Macros.tex}

\input{Environments.tex}

%% Geometrie
\newdimen\lines
\setbox\@tempboxa\hbox{(Programmierung)}
\lines=\ht\@tempboxa
\advance\lines by\dp\@tempboxa

\newlength{\exb}
\settowidth{\exb}{\normalfont x}
\geometry{%
  a4paper,%
  includehead,% (=> head is part of total body)
  ignorefoot,% (=> foot is not part of total body)
  top=3cm,% (top of paper |---| top of total body)
  totalwidth=70\exb,% (width of total body)
  totalheight=215mm,% (height of total body)
  headheight=1\lines,%
  headsep=2.5\lines,%
  foot=4\lines,% (bottom of text body |---| _bottom_ of foot)
  hcentering%
}%

\newcommand{\setauthor}[1]{\author{#1}\def\theauthor{#1}}
\newcommand{\settitle}[1]{\title{#1}\def\thetitle{#1}}

\newcommand{\advisor}[1]{\def\theadvisor{#1}}
\newcommand{\reviewerOne}[1]{\def\thereviewerOne{#1}}
\newcommand{\reviewerTwo}[1]{\def\thereviewerTwo{#1}}
\newcommand{\university}[1]{\def\theuniversity{#1}}
\newcommand{\faculty}[1]{\def\thefaculty{#1}}
\newcommand{\thesistype}[1]{\def\thethesistype{#1}}
\newcommand{\subdate}[3]{\def\thesubday{#1} \def\thesubmonth{#2} \def\thesubyear{#3} }
\newcommand{\city}[1]{\def\thecity{#1}}

\newcommand{\maketitlepage}{
  \begin{titlepage}
    \begin{center}
      \newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
      \begin{minipage}{0.2\textwidth}
%        \includegraphics[draft=false,width=0.9\textwidth]{logo.eps}
      \end{minipage}
      \begin{minipage}{0.7\textwidth}
        \centering \textsc{{\Huge \theuniversity}}

        \centering \textsc{\footnotesize \thefaculty}
      \end{minipage}
      \vspace{1cm}

      \textsc{\thethesistype ~Thesis}\\[0.3cm]
      % Title
      \HRule \\[0.4cm]
      { \Huge \scshape \thetitle \\[0.4cm] }

      \HRule \\[1.5cm]

      % Author and supervisor
      \noindent
      \begin{minipage}{0.4\textwidth}
        \begin{flushleft} \Large
          \emph{Author}\\
          \theauthor
        \end{flushleft}
      \end{minipage}%
      \begin{minipage}{0.4\textwidth}
        \begin{flushright} \Large
          \emph{Advisor} \\
          \theadvisor

        \end{flushright}
      \end{minipage}

      \noindent
      \begin{minipage}{1\textwidth}
        \vspace{7cm}
        \begin{center} \large
          \emph{Reviewers} \\
          \thereviewerOne\\
          \thereviewerTwo
        \end{center}
      \end{minipage}

      \vfill

      {\large Submitted: \thesubday\textsuperscript{th} \thesubmonth~\thesubyear}

    \end{center}
  \end{titlepage}
}

\newcommand{\statementpage}{
~ \vspace*{2cm} ~

\textbf{Eidesstattliche Erkl\"arung}

Ich erkl\"are hiermit an Eides statt, dass ich die vorliegende Arbeit
selbstst\"andig verfasst und keine anderen als die angegebenen Quellen und
Hilfsmittel verwendet habe.

\textbf{Statement in Lieu of an Oath}

I hereby confirm that I have written this thesis on my own and that I
have not used any other media or materials than the ones referred to in
this thesis.


~ \vspace{3cm} ~

\textbf{Einverst\"andniserkl\"arung}

Ich bin damit einverstanden, dass meine (bestandene) Arbeit in beiden
Versionen in die Bibliothek der Informatik aufgenommen und damit
ver\"offentlicht wird.
% \begin{center}
% \Large

\textbf{Declaration of Consent}

I agree to make both versions of my thesis (with a passing grade)
accessible to the public by having them added to the library of the
Computer Science Department.

\vspace*{3cm}

\thecity, \thesubday$^{\text{th}}$ \thesubmonth, \thesubyear

\newpage
}

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:


==> prob_heap_lang.tex <==
	
    \subsection{Instatiation: Probabilistic Heap Lang}

	\begin{align*}
		\infer[wp-choose-uniform]
		{l \neq [] \qquad \forall v \in l.~ \pred~ v \qquad \sum (map~ \potb~ l) \leq \pota \cdot length~ l }
		{\wpP {\pota} {\ChooseUniform{l}} {\potb, \pred}} \qquad
		\infer[wp-tick]
		{c \geq 0 \qquad \later \pred~ ()}
		{\wpP c {\Tick c} {\mathbf{0}, \pred}}
	\end{align*}
	\begin{align*}
		\infer[wp-choose-weighted]
		{l \neq [] \qquad \forall v \in l, \exists r, v'.~ v = (r, v') * r > 0 * \Phi~ v' \qquad \frac{\sum map (\lambda~ (r, v).~ r \cdot \potb~ v)~ l}{\sum map~ fst~ l} \leq p}
		{\wpP \pota {\ChooseWeighted l} {\potb, \Phi}} 
	\end{align*} \todo{make type coersion explicit?}

	\begin{align*}
		\infer[wp-fork]
		{p \geq 0 \qquad \later \pred~ () \qquad \later \wpP p e {\mathbf{0}, True}}
		{\wpP p {Fork~ e} {\mathbf{0}, \pred}}
	\end{align*}

	Furthermore, all rules for deterministic primitives (except for the prophecy) stay valid and can be generalized to an arbitrary nonnegative potential using the rule WP-ADD-POT. \todo{emphasize backwards compatibility}
